struc2vec: Learning Node Representations from Structural Identity

Structural identity is a concept of symmetry in which network nodes are identified according to the network structure and their relationship to other nodes. Structural identity has been studied in theory and practice over the past decades, but only recently has it been addressed with representational learning techniques. This work presents struc2vec, a novel and flexible framework for learning latent representations for the structural identity of nodes. struc2vec uses a hierarchy to measure node similarity at different scales, and constructs a multilayer graph to encode structural similarities and generate structural context for nodes. Numerical experiments indicate that state-of-the-art techniques for learning node representations fail in capturing stronger notions of structural identity, while struc2vec exhibits much superior performance in this task, as it overcomes limitations of prior approaches. As a consequence, numerical experiments indicate that struc2vec improves performance on classification tasks that depend more on structural identity.

==> draft.tex <==


IDEIAS: pegar um vértice de outra rede e "ver" aonde ele fica no espaço latente (interpolação??)

\begin{table}[hbtp]
\caption{Spectral Gap}
\begin{center}
\begin{adjustbox}{max width=\textwidth}

\setlength\extrarowheight{1.5pt}
\begin{tabular}{|c|C{3cm}|C{1.8cm}|}
  \hline 
 \myrowcolour%
   Network & 2th Eigenvalue & Spectral Gap  \\
  \hline 
   Karate espelhado & 0.989 &  \\
  \hline
  \myrowcolour%
   Rede completa Karate espelhado & Layer 0: 0.580 | Layer 1: 0.908 | Layer 2: 0.988 | Layer 3: 0.993 | Layer 4: 0.998 | Layer 5: 0.999 | Layer 6: 0.999 | Layer 7: 0.928 &    \\
  \hline 
   Barbell & 0.998 &  \\
  \hline
  \myrowcolour%
   Rede completa Barbell & Layer 0: 0.853 | Layer 1: 0.997 | Layer 2: 0.999 | Layer 3: 0.999  | Layer 4: 0.999 | Layer 5: 0.999 | Layer 6: 0.999 | Layer 7: 0.999 | Layer 8: 0.999 | Layer 9: 0.999 | Layer 10: 0.999 | Layer 11: 0.999 | Layer 12: 0.986 | Layer 13: 0.0  &   \\
  \hline
\end{tabular}
\end{adjustbox}
\end{center}
\label{tab:tableDegree}
\end{table}







==> structuralequivalence.tex <==


\section{Structural Equivalence}

In a protein-protein interaction (PPI) network proteins exert specific functions based in its structural identity, as catalysis of a cell, for example. In a social network, a collection of actors are joined by pairwise ties. Actors may be individuals or organizations and ties are any type of relationship between two actors, such as friendship, kinship, financial exchange, prestige or influence. 

We can analyze nodes in a networks by looking structures that appears within these networks. For example, we can look at the meaning of cliques or bridges as ways of thinking about and describing how the nodes in a network may be divided into equivalence classes on the basis of their patterns of relations with one another.

Structural identity is a property in function of the structure of a node. We can think that every single node in a network have a structural identity and two nodes are structural equivalents if they share the same structure.

From a sociological perspective, being able to define and analyze data in terms of structural equivalence is important because allow us to make generalization about social behavior and social structure. Social structures like social roles or social positions are studied by sociologists since 1970s~\cite{lorrain1971structural,Sailer1978}. These structures are defined by regularities in the relationships among individuals, not by attributes of them. Because positions or roles are defined by relations among individuals,
we can identify and empirically define social positions using network data. A social position is a collection of actors similarly embedded in a network, for example, judges at different courts occupy the position judge, even though they don't work with each other, or even the same lawyers or attorneys. Two individuals have the same position or role if their pattern
of relationships with other individuals is the same. 

There are three fundamental approaches to constructing measures of network similarity:

\textbf{Structural equivalence:} Two nodes are said to be exactly structurally equivalent if they have exactly the same neighbors, that is, the same relationships to all other nodes. Two nodes must be exactly substitutable in order to be structurally equivalent~\cite{lorrain1971structural}. Because exact structural equivalence is likely to be rare (particularly in large networks), we often are interested in examining the degree of structural equivalence, rather than the simple presence or absence of exact equivalence.

\textbf{Automorphic equivalence:} An isomorphism of graphs $G$ and $H$ is a bijection between the vertex sets of $G$ and $H$ : $ f : V(G) \to V(H) $, such that any two nodes $u$ and $v$ of $G$ are adjacent in $G$ if and only if $f(u)$ and $f(v)$ are adjacent in $H$. An automorphism of a graph $G = (V,E)$ is a permutation $\sigma$ of the vertex set $V$, such that the pair of nodes $(u,v)$ form an edge if and only if the pair $(\sigma(u),\sigma(v))$ also form an edge. That is, it is a graph isomorphism from $G$ to itself. So, a node $u$ is automorphically equivalent to a node $v$ if there exists an automorphism $p$ such that $u = p(v)$, that is, $u$ and $v$ are automorphically equivalent if they have identical ties to equivalent nodes. Two automorphically equivalent nodes share exactly the same label-independent properties, for example, two individuals with exactly the same number of sons, co-workers, etc. Automorphism is extremely difficult to compute and no simple way to relax the concept for application to real world data.

\textbf{Regular equivalence:} Two actors are regularly equivalent if they are equally related to equivalent others. In other words, regularly equivalent nodes are nodes that, while they do not necessarily share neighbors, have neighbors who are themselves similar, for example, two mothers with different numbers of children, etc.

In this work, we are interested in a flexible meaning of structural equivalence, like regular equivalence, because this flexibility allow us to compare nodes of a network in a smooth way, unlike automorphism, where is possible only knows if two nodes are automorphically equivalent or not. 

We'd like to able to discover when two nodes fall in the same equivalence class, and to achieve this we'd like to use structural equivalence. Traditional Approaches to calculate similarity uses euclidean distance or Correlation (Pearson product-moment) applied to thw rows of the adjacent matrix.

We propose a different and novel approach to capture the structural identity of nodes. Let $G = (V , E)$ be a given network, where $V$ are nodes of the network and $E$ its edges $E \subseteq (V \times V)$. Our goal is to learn network feature representations $X \in \mathbb{R}^d$, where $d$ is number of latent dimensions, thats capture the structural identity of nodes in $V$ and obey a relation where a set of embeddings of nodes with exactly or similar roles will be in near positions on the latent space.  

